Interactive Generalized Additive Model and Its Applications in Electric Load Forecasting

Electric load forecasting is an indispensable component of electric power system planning and management. Inaccurate load forecasting may lead to the threat of outages or a waste of energy. Accurate electric load forecasting is challenging when there is limited data or even no data, such as load forecasting in holiday, or under extreme weather conditions. As high-stakes decision-making usually follows after load forecasting, model interpretability is crucial for the adoption of forecasting models. In this paper, we propose an interactive GAM which is not only interpretable but also can incorporate specific domain knowledge in electric power industry for improved performance. This boosting-based GAM leverages piecewise linear functions and can be learned through our efficient algorithm. In both public benchmark and electricity datasets, our interactive GAM outperforms current state-of-the-art methods and demonstrates good generalization ability in the cases of extreme weather events. We launched a user-friendly web-based tool based on interactive GAM and already incorporated it into our eForecaster product, a unified AI platform for electricity forecasting.

==> 2_bak.tex <==
\section{Related Work}
We first review the current state-of-the-art of electric load forecasting techniques, and then present recent works pertaining to GAMs their properties in ELF.

Electric load usually involves nonlinearity modeling and exhibits seasonality patterns that change over time due to factors like weather changes~\cite{wang2016electric}, the economy drifts and holiday effect~\cite{dryar1944effect}. The electricity demand data, compared to sales data, can be of greater granularity temporally and spatially~\cite{hong2016probabilistic}. Based on the sophisticated nature of ELF, neural network is applied. In late 1990s, the Electric Power Research Institute sponsored a project to see about a short-term load forecasting system based on neural networks~\cite{khotanzad1998annstlf}. The resulting products are still being used by many power companies today. Later, a large body of literature has developed and applied deep learning models including LSTM-RNN~\cite{he2017load}, RBM~\cite{li2017building}, CNN~\cite{zahid2019electricity} and more recently, transformer-based network~\cite{zhou2022fedformer,chen2022learning}.  Despite of the strong fitting power, deep learning architectures often suffer from over-fitting due to multiple layers~\cite{shi2017deep} and not well-interpretable to human. 

Neural network is not the dominating methodology. In fact, based on the Global Energy Forecasting Competition (GEFCom) held in 2012, 2014 and 2017~\cite{hong2014global,hong2016probabilistic,hong2019global}, the majority of the top-ranked teams consider statistical methods including Gradient Boosting Machines (GBM), quantile regression and Generalized Additive Models. These methods have achieved competitive test accuracy. GBM framework (including XGBoost~\cite{chen2016xgboost}, CatBoost~\cite{prokhorenkova2018catboost}, LightGBM~\cite{ke2017lightgbm}), particularly, has enjoyed tremendous popularity in the load forecasting community~\cite{landry2016probabilistic,huang2016semi,smyl2019machine}, for GBM can deal with seasonality as well as auto-correlation and the prediction follows the real load at most of the time. By implementing aggregate algorithm over decision trees, GBM gains explainability for the ensemble~\cite{delgado2022implementing}. However, it is reported that GBM may not predict well at the high loads~\cite{abbasi2019short}. This is because the set of high loads data points are under-represented and overlooked by the training process. Also, extrapolation is tough for such tree-based ensemble learners~\cite{meyer2021predicting}, thus the out-of-the-box prediction may fail when the data contains features in which the extrapolation is not implicit. 


Among the top-ranked teams in GEFCom2012, 2014 and 2017, many proposed techniques with or assembled with a highly explainable Generalized Additive Model (GAM)~\cite{hastie2017generalized} to tackle with extreme weather conditions and volatile, fluctuating load~\cite{nedellec2014gefcom2012,gaillard2016additive,sigauke2017forecasting}. In real application of power system, GAM has been widely adopted. For example, projects sponsored by Australian Energy Market Operators~\cite{fan2011short,fan2012forecasting} have developed a modified semi-parametric version of GAM. Their work is now in the package called Monash Electricity Forecasting Model (MEFM). An extension of GAM with LASSO and tensor product interactions have also demonstrated its power in forecasting South Africa data~\cite{sigauke2017forecasting}, making it a useful tool for system operators in power utility companies. 

Compared to neural network and gradient boosting framework, GAM is adored by the industry for the following reasons. First, it identifies and characterizes nonlinear regression effects~\cite{hastie2009elements} and is able to jump the accuracy hurdles. Under certain scenarios in ELF, GAM outperforms other methods~\cite{gaillard2016additive}. Indeed, GAM describes relationship between factors in a much simpler way. Though some level of sophistication is necessary to achieve high accuracy, the industry may not need the most high accuracy anyway. Those aforementioned successful projects have found a good balance between simplicity and accuracy. Second, GAM is simple enough for human experts to read each component of the model, recognize which the significant predictors are and how a GAM works~\cite{hegselmann2020evaluation}. Concretely, GAM is explainable because the effect of each factor on the prediction can be visualized in a graph. Thus humans can work on the follow-up feedback, such as model-debiasing~\cite{tan2018distill}, or potentially, refining the under-fitting parts. 





 1. fast algorithm \cite{lou2013accurate}2. application: 1. general, FLAM \cite{petersen2016fused} 2: editable GAM-microsoft \cite{wang2022interpretability}GAM Changer, the first
interactive system to help domain experts and data scientists easily and responsibly edit Generalized Additive Models (GAMs) and fix problematic patterns. 










==> 3_bak <==
\section{Problem Formulation}
\emph{This paragraph can be moved to the introduction section}
We consider the electric load forecasting under extreme whether event.
As the extreme whether events happen rarely in the history, few data about the electric load can be collected.
Fortunately, some domain knowledge from the experts can alleviate the lack of data about the electric load under extreme whether event.
For example, in the summer, when the temperature 
increase from 36 to 37  Celsius degree, the 
electric load increase much more than that 
when he temperature 
increase from 34 to 35 Celsius degree, as more air conditioners are opened when the temperature increase.
Nevertheless, when temperature is too high (say above 41 Celsius degree), most air conditioners have been working,
electric load saturation happens,
increasing temperature only leads to few load rising.
Thus we can conclude that when the temperature is above about
27 and below about 41 Celsius degree, the load is convex with respect to temperature and
when temperature is above about 41 Celsius degree the electric load is concave with respect to temperature.

In electric load forecasting, due to the lack of training data under extreme weather conditions and the consideration of interpretability, it is very helpful to incorporate domain knowledge from expert  

These domain knowledge have two key properties. Firstly, these knowledge
are high-level knowledge, i.e., we can only know the trend of
load with respect to some factors, and can not know the exactly what value does the load take when given the values of part of factors.
Secondly, even the high-level knowledge, one can not exactly determinate
the range of the knowledge applied, such as even experienced experts can not exactly tell on which temperature level the load saturation happens.
Thus to incorporate these rough and high-level domain knowledge, 
we propose to build an interactive generalized additive model (GAM), where the high-level domain
knowledge is formulate as constraints, the model is able to provide hint to users, and the users are allowed to try different constraints
and get the results in time.
Let $\boldsymbol{x}_t$ be a collection of $M$ features at time $t$, which consist of features about whether, time and electric load in history, and $y_t$ be the electric load in time $t$, GAMs formulate $y_t$ as 
the summation of the individual effects of $\{x_{t}^i\}_{i=1}^M$,
i.e.,
\begin{align}
y_t \approx \sum_{i=1}^M f_i(x_t^i)
\end{align}
where
$x_{t}^i$ denotes the $i$th feature of $\boldsymbol{x}_t$, $f_i(\cdot)$ 
denotes the shape function of the $i$th feature.
To incorporate the domain knowledge, given a dataset $\{(\boldsymbol{x}_t,y_t)\}_{t=1}^N$, we aim to solve the following
problem
\begin{align}
\min_{\{f_i\}}&\quad\sum_{t=1}^{N} w_i\left(y_t-\sum_{i=1}^M f_i(x_t^i)\right)^2\\
\text{s.t.}&\quad f_i\in \mathcal{A}_i\quad \forall i=1\dots M
\end{align}
where $w_t$ denotes the weight of $t$th sample, $\mathcal{A}_i$ denotes the set consists of all shape functions satisfy the constraints added by user.
We note that although we write the constraints in the formulation stage, actually, these constraints are added in
interactive manner, i.e., the constraints are added after the model is trained, and once the constraints added, the model is adjusted to fit these constraints.

We discuss the sets ${\mathcal{A}_i}$. As ${\mathcal{A}_i}$ is formed by the combination of constraints, thus we only needs to consider the type of these constraints. We perform
a survey among the experts on electric power companies, and 
find that most domain knowledge can be classified as four types, i.e., the electric load is monotone increase, monotone decrease, convex, and concave with respective to some
factors at some ranges.
Thus we only consider these four types constraints in this paper. It is notable that the convex combination of two 
monotone increase shape functions is also a monotone increase
function, and this property is also hold for monotone decrease, convex, and concave functions.
Then it is readily to see that ${\mathcal{A}_i}$
are convex sets, and we will show that this critical 
property empower us to develop efficient methods
to learn a set of shape functions to satisfy these constraints.

When extreme whether events happens,
some whether features are out of the
range of its history values. Thus,
good generalization on out of range data is desired. Usually, for the electric load forecasting problem,
the trend of the affect of factors
is smooth. For instance, if raising
the temperature from 38 to 39 Celsius
degree leads to 10MW electric load 
increasing, then raising
the temperature from 39 to 40 Celsius
degree, electric load increasing
is also around 10MW.
To utilize this property, we further
restrict the shape function $f_i(\cdot)$ being
piecewise linear.



==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

